Online Multilinear Dictionary Learning

A method for online tensor dictionary learning is proposed. With the assumption of separable dictionaries, tensor contraction is used to diminish a $N$-way model of $\mathcal{O}\left(L^N\right)$ into a simple matrix equation of $\mathcal{O}\left(NL^2\right)$ with a real-time capability. To avoid numerical instability due to inversion of sparse matrix, a class of stochastic gradient with memory is formulated via a least-square solution to guarantee convergence and robustness. Both gradient descent with exact line search and Newton's method are discussed and realized. Extensions onto how to deal with bad initialization and outliers are also explained in detail. Experiments on two synthetic signals confirms an impressive performance of our proposed method.

==> Sects/5_analyze.tex <==
\section{Performance Analysis}

==> Sects/8_append.tex <==
\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.

==> Sects/9_acknowledge.tex <==
% use section* for acknowledgement
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi

The authors would like to thank...

==> Sects/online_wrong_note.tex <==
The proposed OMDL will be derived in the fashion similar to~\cite{Yim2017}. Let \textit{a priori} gradient matrix $\mathbf{G}_{t|t-1}^{(n)}$ be defined as
\begin{equation}
\label{eq:19}
\mathbf{G}_{t|t-1}^{(n)}\triangleq\left.\frac{\partial\mathcal{J}_t^{(n)}}{\partial\boldsymbol{\Psi}^{(n)}}\right\vert_{\boldsymbol{\Psi}^{(n)}=\boldsymbol{\Psi}_{t-1}^{(n)}}=\boldsymbol{\Psi}_{t-1}^{(n)}\mathbf{R}_t^{(n)}-\mathbf{P}_t^{(n)}.
\end{equation}
Then, the expression of mode-$n$ dictionary update becomes
\begin{equation}
\label{eq:20}
\boldsymbol{\Psi}_t^{(n)}=\boldsymbol{\Psi}_{t-1}^{(n)}+\alpha^{(n)}_t\mathbf{D}_t^{(n)}, %\bm{\mathcal{P}}_{\mathbi{C}^{(n)}}\left( \right)
\end{equation}
where the step size $\alpha^{(n)}_t>0$ are any appropriate positive scalar and the descent direction $\mathbf{D}_t^{(n)}$ are any matrix which ensures $\mathcal{J}_t(\boldsymbol{\Psi}_t^{(n)})<\mathcal{J}_t(\boldsymbol{\Psi}_{t-1}^{(n)}) \ \forall t$ and, as a result, satisfies
\begin{equation}
\label{eq:21}
{\left\langle \mathbf{D}_t^{(n)},\mathbf{G}_{t|t-1}^{(n)}\right\rangle}_F<0.
\end{equation}
${\langle\cdot,\cdot\rangle}_F$ denotes the Frobenius inner product and $\alpha^{(n)}_t$ can be analytically obtained by the exact line search in which $\partial\mathcal{J}_t(\boldsymbol{\Psi}_t^{(n)})/\partial\alpha^{(n)}_t$ is set to zero, yielding
\begin{equation}
\label{eq:22}
\alpha^{(n)}_t=\left. - {\left\langle \mathbf{D}_t^{(n)},\mathbf{G}_{t|t-1}^{(n)}\right\rangle}_F \middle/ {\left\langle \mathbf{D}_t^{(n)},\mathbf{H}_{t|t}^{(n)}\right\rangle}_F \right.
\end{equation}
where
\begin{equation}
\label{eq:23}
\mathbf{H}_{t|t}^{(n)}=\mathbf{D}_t^{(n)}\mathbf{R}_t^{(n)}.
\end{equation}
Not that~\eqref{eq:20} does not guarantee $\boldsymbol{\Psi}_t^{(n)}\subset\mathbi{C}^{(n)}, \ \forall t$, the projection operator $\bm{\mathcal{P}}_{\mathbi{C}^{(n)}}$ is used on $\boldsymbol{\Psi}_t^{(n)}$ such that
\begin{equation*}
\boldsymbol{\Psi}_t^{(n)} \leftarrow \bm{\mathcal{P}}_{\mathbi{C}^{(n)}}\left( \boldsymbol{\Psi}_t^{(n)} \right)\subset\mathbi{C}^{(n)}.
\end{equation*}
For simplicity, this paper consider the case where the convex set $\mathbi{C}^{(n)}$ is a linear map which conserves a space spanned by the dictionary atoms i.e. the column space. We can express such a map with a diagonal matrix $\boldsymbol{\Pi}_t^{(n)}\in\mathbb{R}^{L_{n}\times L_{n}}$ and such that
\begin{equation}
\label{eq:24}
\boldsymbol{\Psi}_t^{(n)} \leftarrow \boldsymbol{\Psi}_t^{(n)}\boldsymbol{\Pi}_t^{(n)}.
\end{equation}
An example of $\mathbi{C}^{(n)}$ can be a unit column norm where each diagonal element in $\boldsymbol{\Pi}_t^{(n)}$ equals the inverse
of the 2-norm of the corresponding column of $\boldsymbol{\Psi}_t^{(n)}$. However, the mapping in~\eqref{eq:24} will require $\mathbf{R}_t^{(n)}$, $\mathbf{P}_t^{(n)}$ and $\mathbf{G}_{t|t-1}^{(n)}$ to be adjusted accordingly, complicating the algorithm and contributing to large complexity in each iteration. Since $\boldsymbol{\Pi}_t^{(n)}$ does not alter the column space of $\boldsymbol{\Psi}_t^{(n)}$, the desired algebraic structure is maintained. Therefore,~\eqref{eq:24} can be skipped completely from the algorithm and performed only to display the dictionary at the required time instant.

Now, to reuse past calculations recursively, \textit{a posteriori} gradient matrix $\mathbf{G}_{t|t}^{(n)}$ and an instantaneous gradient matrix $\mathbf{F}_t^{(n)}$ are defined respectively as
\begin{equation}
\label{eq:25}
\mathbf{G}_{t|t}^{(n)}\triangleq\left.\frac{\partial\mathcal{J}_t^{(n)}}{\partial\boldsymbol{\Psi}^{(n)}}\right\vert_{\boldsymbol{\Psi}^{(n)}=\boldsymbol{\Psi}_t^{(n)}}=\boldsymbol{\Psi}_t^{(n)}\mathbf{R}_t^{(n)}-\mathbf{P}_t^{(n)}
\end{equation}
\noindent and
\begin{equation}
\label{eq:26}
\mathbf{F}_t^{(n)}=\boldsymbol{\Psi}_{t-1}^{(n)}\mathbf{S}_t^{(n)}-\mathbf{Q}_t^{(n)}.
\end{equation}
After some manipulation, we arrive at the dual recursion between $\mathbf{G}_{t|t-1}^{(n)}$ and $\mathbf{G}_{t|t-1}^{(n)}$:
\begin{equation}
\label{eq:27}
\mathbf{G}_{t|t-1}^{(n)}=\lambda\mathbf{G}_{t-1|t-1}^{(n)}+\mathbf{F}_t^{(n)},
\end{equation}
\begin{equation}
\label{eq:28}
\mathbf{G}_{t|t}^{(n)}=\mathbf{G}_{t|t-1}^{(n)}+\alpha^{(n)}_t\mathbf{H}_{t|t}^{(n)}.
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Conjugate Gradient Descent (CGD)}
As one of the most efficient first-order solvers of a quadratic-form equation, the CGD method is utilized to derive our method here. Although successfully implemented in the context of offline MDL~\cite{Hawe2013}, the conjugacy property can no longer be maintained in the online setting where the statistics of $\mathbf{R}_t^{(n)}$ varies. Rather, only the intermediate conjugacy is employed to make possible the recursive algorithm, and in the similar spirit to the \textbf{Definition 1} in~\cite{Yim2017}, a descent direction $\mathbf{D}_t^{(n)}$ is \textit{Markov} conjugate if, for any instant $t$,
\begin{equation}
\label{eq:29}
\textnormal{Tr}\left(\mathbf{D}_{t-1}^{(n)}\mathbf{R}_t^{(n)}{\mathbf{D}_t^{(n)}}^T\right)=0, \ \forall n\in\mathbi{N}.
\end{equation}
This definition makes use of only one degree of freedom and consequently yields a desirably simple expression of the conjugate direction as
\begin{equation}
\label{eq:30}
\mathbf{D}_{t}^{(n)}=-\mathbf{G}_{t|t-1}^{(n)}+\beta_t^{(n)}\mathbf{D}_{t-1}^{(n)}.
\end{equation}
The constant $\beta_t^{(n)}$ is calculated by pre-multiplying the transpose of~\eqref{eq:30} with $\mathbf{D}_{t-1}^{(n)}\mathbf{R}_t$ and substituting into~\eqref{eq:29}, giving
\begin{equation}
\label{eq:31}
\beta_t^{(n)}=\left.{\left\langle \mathbf{D}_{t-1}^{(n)},\mathbf{V}_t^{(n)}\right\rangle}_F \middle/ {\left\langle \mathbf{D}_{t-1}^{(n)},\mathbf{H}_{t|t-1}^{(n)}\right\rangle}_F \right.,
\end{equation}
where
\begin{equation}
\label{eq:32}
\mathbf{H}_{t|t-1}^{(n)}=\mathbf{D}_{t-1}^{(n)}\mathbf{R}_t^{(n)}
\end{equation}
\begin{equation}
\label{eq:33}
\mathbf{V}_t^{(n)}=\mathbf{G}_{t|t-1}^{(n)}\mathbf{R}_t^{(n)}
\end{equation}
It is shown in Appendix I that $\mathbf{D}_{t}^{(n)}$ also satisfies~\eqref{eq:21}, thereby a descent direction. Eventually, the dual recursion of `gain matrices' is given by
\begin{equation}
\label{eq:34}
\mathbf{H}_{t|t-1}^{(n)}=\lambda\mathbf{H}_{t-1|t-1}^{(n)}+\mathbf{D}_{t-1}^{(n)}\mathbf{S}_t^{(n)},
\end{equation}
\begin{equation}
\label{eq:35}
\mathbf{H}_{t|t}^{(n)}=-\mathbf{V}_t^{(n)}+\beta_t^{(n)}\mathbf{H}_{t|t-1}^{(n)}.
\end{equation}

Another possibility is to opt for a second-order or Newton's direction. From the cost function in~\eqref{eq:16} and gradient matrix in~\eqref{eq:19}, a quasi-Newton alternative of $\mathbf{D}_t^{(n)}$ would be in the form
\begin{equation}
\label{eq:36}
\mathbf{D}_t^{(n)}=-\mathbf{G}_t^{(n)}\boldsymbol{\Upsilon}_{t-1}^{(n)},
\end{equation}
where $\boldsymbol{\Upsilon}_{t-1}^{(n)}$ is the approximate of ${\mathbf{R}_{t-1}^{(n)}}^{-1}$. A variety of quasi-Newton methods can be utilized to update $\boldsymbol{\Upsilon}_t^{(n)}$ For example, the BFGS method will render the iterative correction of $\boldsymbol{\Upsilon}_t^{(n)}$ given in~\eqref{eq:28}
\begin{figure*}[!b]
\normalsize
\hrulefill
\begin{equation}
\label{eq:37}
\boldsymbol{\Upsilon}_t^{(n)}=\left( \mathbf{I}-{\boldsymbol{\Xi}_t^{(n)}}^T\mathbf{H}_{t|t}^{(n)} \right)\boldsymbol{\Upsilon}_{t-1}^{(n)}\left( \mathbf{I}-{\mathbf{H}_{t|t}^{(n)}}^T\boldsymbol{\Xi}_t^{(n)} \right)+{\mathbf{D}_t^{(n)}}^T\boldsymbol{\Xi}_t^{(n)}
\end{equation}
\end{figure*}
where
\begin{equation}
\label{eq:38}
\boldsymbol{\Xi}_t^{(n)}={\left( \mathbf{D}_t^{(n)}{\mathbf{H}_{t|t}^{(n)}}^T \right)}^{-1}\mathbf{D}_t^{(n)}.
\end{equation}
We will not proceed further to elaborate on the quasi-Newton method and will let it be open research for any interested readers. To this end, we shall settle on the CGD method.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Decimating Erroneous Dictionaries}
Since the sparse coefficients $\mathbfcal{S}_t$ at initial iterations would be far off its actual values due to the randomly initialized dictionaries $\boldsymbol{\Psi}_0^{(n)}$, $\mathbf{R}_t^{(n)}$, also thereby $\mathbf{G}_{t|t-1}^{(n)}$, will be biased and $\boldsymbol{\Psi}_t^{(n)}$ will be incorrectly adjusted. It is thus plausible to eliminate the effect of $\boldsymbol{\Psi}_t^{(n)}$ distant from current iteration.

\medskip
\noindent \textit{A. Sliding Window}
\medskip

The most straightforward means to alleviate the mismatch from far past data is to impose the cost function $\mathcal{J}_t^{(n)}$ to intake $T$ most \textit{recent} data i.e. when the next data arrives, the data window of size $T$ slides through and selects the data from the current $t$ down to $t-T+1$. As a result, $\mathcal{J}_t^{(n)}$ in~\eqref{eq:11} becomes
\begin{equation}
\label{eq:39}
\mathcal{J}_t^{(n)}\triangleq{\sum\limits_{\tau=t-T+1}^t}w_{\tau}\left\Vert \mathbfcal{X}_{\tau}-\mathbfcal{\tilde{S}}_{\tau}^{(n)}\times_n\boldsymbol{\Psi}^{(n)}\right\Vert _{F}^{2}.
\end{equation}
By~\eqref{eq:39}, most equations derived above remain unchanged except that $\mathbf{S}_t^{(n)}$ and $\mathbf{Q}_t^{(n)}$ will now become \textit{windowed} arriving data and take the following form:
\begin{equation}
\label{eq:40}
\mathbf{S}_{t}^{(n)}=\left\{ \begin{array}{cl}
\tilde{\mathbf{S}}_t^{(n)}-\mathit{\Lambda}_{t-T}\tilde{\mathbf{S}}_{t-T}^{(n)} & t > T \\
\tilde{\mathbf{S}}_t^{(n)} & t \leq T 
\end{array}\right.
\end{equation}
and
\begin{equation}
\label{eq:41}
\mathbf{Q}_{t}^{(n)}=\left\{ \begin{array}{cl}
\tilde{\mathbf{Q}}_t^{(n)}-\mathit{\Lambda}_{t-T}\tilde{\mathbf{Q}}_{t-T}^{(n)} & t > T \\
\tilde{\mathbf{Q}}_t^{(n)} & t \leq T 
\end{array}\right.
\end{equation}
where $\mathit{\Lambda}_{t-T}={\prod_{\tau=1}^T}w_{\tau}$ and $w_{\tau}={\lambda}^{t-\tau}$. To select the proper size of sliding window, its effect on \textit{a priori} gradient needs to be pointed out. In the rank-$1$ LMS-like method~\cite{Aharon2008}, only one most recent sample is used to estimate $\mathbf{G}_{t|t-1}^{(n)}$, thereby ``rank-$1$". In~\cite{Mairal2010}, \textit{a priori} gradient is approximated by all past information, making it possibly ``full-rank" and a better estimate. As it will take some time for those erroneous data to vanish completely even with forgetting factor and the maximal rank the matrix $\mathbf{G}_{t|t-1}^{(n)}$ can attain is $L_n$, then $T > L_n$ will guarantee \textit{a priori} gradient to be full-rank (under assumption that the rank of $\mathbf{F}_t^{(n)}\, \forall t$ is at least $1$).

\begin{algorithm}
\label{alg:1}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{DoWhile}{do}{while}

\Input{$x_n$, $y_n$, $M$, $\lambda$, $\epsilon$, $\delta$ and \textit{update scheme}}
\Output{$\hat{y}_n$ and $\mathbf{w}^{op}$}
 Initialize $\mathbf{w}_0=\mathbf{d}_0=\mathbf{g}_{0|0}=\mathbf{h}_{0|0}=\mathbf{0}$ and $\mathbf{R}_0=\mathbf{\underline{0}}$\;
 $n=0$\;
 \DoWhile{${\| e_n \|} > \delta$ \textnormal{or} $n=N$}{
  $t=t+1$\;
  
  Update $\mathbf{S}_t^{(n)}$ and $\mathbf{Q}_t^{(n)}$ according to~\eqref{eq:40} and~\eqref{eq:41}\;
  $\mathbf{F}_t^{(n)}=\boldsymbol{\Psi}_{t-1}^{(n)}\mathbf{S}_t^{(n)}-\mathbf{Q}_t^{(n)}$\;
  $\hat{y}_n-{(\mathbf{w}_{n-1})}^H\mathbf{q}_n$\;
  $e_n=y_n-\hat{y}_n$\;
  
  $\mathbf{R}_t^{(n)}=\lambda_{t-1}\mathbf{R}_{t-1}^{(n)}+\mathbf{S}_t^{(n)}$\;
  $\mathbf{G}_{t|t-1}^{(n)}=\lambda_{t-1}\mathbf{G}_{t-1|t-1}^{(n)}+\mathbf{F}_t^{(n)}$\;
  $\mathbf{V}_t^{(n)}=\mathbf{G}_{t|t-1}^{(n)}\mathbf{R}_t^{(n)}$\;
  
  $\mathbf{H}_{t|t-1}^{(n)}=\lambda_{t-1}\mathbf{H}_{t-1|t-1}^{(n)}+\mathbf{D}_{t-1}^{(n)}\mathbf{S}_t^{(n)}$\;
  $\beta_t^{(n)}=\left.{\left\langle \mathbf{D}_{t-1}^{(n)},\mathbf{V}_t^{(n)}\right\rangle}_F \middle/ {\left\langle \mathbf{D}_{t-1}^{(n)},\mathbf{H}_{t|t-1}^{(n)}\right\rangle}_F \right.$\;
  $\mathbf{D}_{t}^{(n)}=-\mathbf{G}_{t|t-1}^{(n)}+\beta_t^{(n)}\mathbf{D}_{t-1}^{(n)}$\;
  $\mathbf{H}_{t|t}^{(n)}=-\mathbf{V}_t^{(n)}+\beta_t^{(n)}\mathbf{H}_{t|t-1}^{(n)}$\;
  
  $\alpha^{(n)}_t=\left. - {\left\langle \mathbf{D}_t^{(n)},\mathbf{G}_{t|t-1}^{(n)}\right\rangle}_F \middle/ {\left\langle \mathbf{D}_t^{(n)},\mathbf{H}_{t|t}^{(n)}\right\rangle}_F \right.$\;
  $\boldsymbol{\Psi}_t^{(n)}=\boldsymbol{\Psi}_{t-1}^{(n)}+\alpha^{(n)}_t\mathbf{D}_t^{(n)}$\;
  $\mathbf{G}_{t|t}^{(n)}=\mathbf{G}_{t|t-1}^{(n)}+\alpha^{(n)}_t\mathbf{H}_{t|t}^{(n)}$\;
 }
 $\mathbf{w}^{op}=\mathbf{w}_n$.
\caption{Online Mode-Wise Dictionary Update}
\end{algorithm}

\medskip
\noindent \textit{B. Adaptive Forgetting Factor}
\medskip

Instead of static $\lambda$, it can be made adaptive, i.e. $\lambda_t$ to even benefit the convergence. As the iterations grow, the dictionaries would get closer to their real values. It is hence sensible to begin with a small value of $\lambda_t$ - to quickly forget the not so good dictionaries - and then gradually increase $\lambda_t$ towards $1$ - to remember more the more accurate dictionaries. There are several adaptive schemes for $\lambda_t$ e.g. linear, quadratic, cubic, exponential, hyperbola, etc. Here, we resort to a quartic function which sets $\lambda_t$ to increase from $\lambda_{0}$ to $1$ in \textit{pre-defined} $\tau$ iterations
\begin{equation}
\label{eq:42}
\lambda_t=\begin{cases}
1-(1-\lambda_{0})(1-t/\tau)^{4} & \textnormal{if} \ t<\tau\\
1 & \textnormal{if} \ t \geq \tau
\end{cases}
\end{equation}
Additionally, even though the dictionaries get closer to their real values after some iterations, the samples may not be consistent with the dictionaries in the presence of outliers which could make the error of the arriving data undesirably large. The influence of the arriving data can be curbed by tuning it with some \textit{weight} $\omega_t$ which modifies ~\eqref{eq:42} to yield a combined adaptive forgetting factor
\begin{equation}
\label{eq:43}
\lambda_t\leftarrow\lambda_t\omega_t,
\end{equation}
where $\omega_t$ should be \textit{disproportionate} to the correctness of the corresponding dictionary, for instance, \begin{equation}
\label{eq:44}
\omega_t=\left( 1+ \left[ \left\Vert \mathbf{F}_t^{(n)} \right\Vert_{F} \middle/ \sqrt{\textnormal{Tr}\left(\mathbf{S}_t^{(n)}\right)}\right] \right)^{-1}
\end{equation}

